Highly Accurate Disease Diagnosis and Highly Reproducible Biomarker Identification with PathFormer

Biomarker identification is critical for precise disease diagnosis and understanding disease pathogenesis in omics data analysis, like using fold change and regression analysis. Graph neural networks (GNNs) have been the dominant deep learning model for analyzing graph-structured data. However, we found two major limitations of existing GNNs in omics data analysis, i.e., limited-prediction (diagnosis) accuracy and limited-reproducible biomarker identification capacity across multiple datasets. The root of the challenges is the unique graph structure of biological signaling pathways, which consists of a large number of targets and intensive and complex signaling interactions among these targets. To resolve these two challenges, in this study, we presented a novel GNN model architecture, named PathFormer, which systematically integrate signaling network, priori knowledge and omics data to rank biomarkers and predict disease diagnosis. In the comparison results, PathFormer outperformed existing GNN models significantly in terms of highly accurate prediction capability ( 30% accuracy improvement in disease diagnosis compared with existing GNN models) and high reproducibility of biomarker ranking across different datasets. The improvement was confirmed using two independent Alzheimer's Disease (AD) and cancer transcriptomic datasets. The PathFormer model can be directly applied to other omics data analysis studies.

==> 3_method.tex <==
In this section, we introduce the proposed PathFormer model. For notation convenience, we first define some basic concepts that will be used in the graph analysis and graph signal processing. We consider a graph $G=(V,E,X)$ where $V={1,2,…,n}$ is the node set of size $N=|V|$, $E \in V  \times V$ is the edge set, and $X \in \mathbb{R}^{n \times d}$ is the d-dimensional node feature tensor with a feature dimension of $d$. For each node $i$ in a graph $G$, we denote by $N(i)= \{j \in V | (i,j) \in E \}$ the neighboring node set of node i, and we denote by $D(j)$ the dependent node set of node j such that there exists a path from node i to node j iff $j \in D(j)$.

\subsection{Overview of PathFormer Model}

The gene network analysis problem is essentially a graph learning task. Learning based graph classification is usually achieved by three steps: (1) iteratively updating node feature vectors through message passing (graph convolution) layers; (2) summarizing final node feature vectors as a graph vector/representation through a readout layer; (3) predicting the graph label based on graph representation through a standard MLP (multiple layer perceptron). Following this scheme, our PathFormer model introduces a novel graph convolution layer, PathFormer encoder layer, to tackle the effective limitation and over-squashing problem. In addition, PathFormer also proposes two interpretation machines which inject the interpretability into the readout layer to generate the graph representation/vector. Figure 3 (b) illustrates the overall architecture of proposed PathFormer model, where the PathFormer encoder layer, interpretation machines, and MLP can be trained together in an end-to-end fashion.

\subsection{Prior-canonical-label top-K sorting}

In the gene-network prediction problems, gene networks (i.e. graphs) share an universal canonical labeling property that provides finer inductive bias than general graphs such that gene index (i.e., gene name) itself encodes the ‘position’ of a node and can be used to distinguish genes. The gene indexes itself can serve as canonical labels, which implicitly solve the challenging graph canonization problem in the situation. That is, using gene index as gene label will provides the canonical form of input gene network.
To facilitate the core gene sub-network detection task, we propose to model the importance distribution of genes based on the prior canonical labels $\mathbb{T}$, and train it in an end-to-end fashion. Then, we can implement the top-K sorting as Sortpool. Here we assign a trainable weight $w_{t}$ to each canonical label in $\mathbb{T}$. Then, for each input graph, the gene importance is computed as:
\begin{align*}
    \epsilon(v|\mathbb{T}) = w_{p(v)} \ \ \forall \ v \in V 
\end{align*}
Then the distribution of gene importance can be computed by normalizing $\{\epsilon(v|\mathbb{T}) | v \in V\}$, and we can get the top-k indexes $\textit{idx}$. Let $\epsilon$ be the normalized gene importance distribution, then we get the corresponding weights $\epsilon_{G} = \epsilon[\textit{idx}]$ as a multiplier to the input to the first pathformer encoder layer.

\begin{figure}[t]
\begin{center}
%\vskip -0.15in
\centerline{\includegraphics[width=0.9\textwidth]{archi_overall.pdf}}
\vspace{-10pt}
\caption{Architecture overview. (a) introduces the basic component, PathFormer encoder layer. (b) illustrates that the PathFormer model consists of a stack of PathFormer encoder layers and two subsequent interpretation mechanisms.}
\vskip -0.18in
\label{fig:1}
\end{center}
\end{figure}




\subsection{PathFormer Encoder Layer }

The proposed PathFormer encoder layer (graph convolution layer) resorts to the attention mechanism to address the over-squashing problem. An Intuitive choice for implementing the attention-based graph convolution operation is to use the self-attention mechanism in the standard Transformer model, As (self)-attention based information propagation models (such as Transformer) have been proven to be efficient for over-squashing problem [21]. However, self-attention mechanism equivalently treats genes with same profile expression, which ignores the topology and pathway information in the attention scores and makes it difficult to design downstream interpretation method for extracting biological meaningful information. In addition, the self-attention mechanism also fails to incorporate the inductive bias that each gene only appears at most once in each gene network and the same pair of nodes’ connectivity is consistent across gene networks. 

To address these drawbacks, our PathFormer encoder layer introduces three innovative design aspects to improve the standard self-attention mechanism (SAM) in gene network analysis. (1) To incorporate topology information in the attention matrix of attention mechanism, GNNs are used to replace the linear layer in SAM when computing the key matrix K, and query matrix Q. (2) To encode pathway information in the input gene network, we assume that genes interact with each other through the shortest path between them. Then PathFormer encoder layer extracts pathways between genes and uses MLP to learn the pathway correlation. (3) Gene indexes are used as the positional encodings. As each gene at most appears once in each gene network, the gene index can be used to uniformly distinguish genes in the same graph, indicating that using gene indexes as the additional features can provably find the canonical form of input gene network, which inherently solves the graph canonization problem and maximize the expressive power. 

Figure 3 (a) illustrates the architecture of PathFormer encoder layer. We denote by the input to the k-th PathFormer encoder layer $H^k=(h_1^k,h_2^k,…,h_n^k)$, where vector $h_v^k$ is obtained by concatenating the gene feature $z^{k-1)} (v)$ from the last layer and the one-hot encoding of gene index (i.e. canonical label) i(v). In the first layer, $z^0 (v)$ is the initial gene expression profile. Then, in the proposed global attention mechanism, the query matrix $Q^k$  and key matrix $K^k$  are computed with GNNs, while value matrix $V^k$ is computed with a linear projection layer (i.e. LP),   
\begin{align*}
    Q^k &= \textit{GNN}^{Q}(H^k, A) \\
    K^k &= \textit{GNN}^{K}(H^k, A) \\
    V^k &= \textit{LP}(H^k) 
\end{align*}
As the strategy of using gene indexes as positional encoding provides equal expressivity as directly distinguishing the canonical form of input gene network, adding $i(v)$ in the input $h_v^k$ will enable GNNs to distinguish all different gene network architectures. As the gene index of the same gene and the connections of same gene pair are shared among different gene networks, the proposed positional encoding method also has good generalization ability to be applied to unseen gene networks.

Some recent research in Bioinformatics [] indicate that the personalized biomarkers may varies across different patients/samples, which makes the population-based analysis fail to detect these biomarkers. However, many personalized biomarkers from different patients are observed to formulate signaling pathways, thus pathway analysis shows huge potential in revealing the mechanism of disease phenotypes. Following this inspiration, we also propose to incorporate pathway information in the global attention mechanism. Specifically, for each pair of gene (i.e. gene i and gene j), we extract the shortest path ($\mathbb{SP}_{i,j}$) between them. Each shortest path is represented as the sequence of gene features and the gene index. Then the pathway correlation matrix T is computed through a MLP and is used as a bias term to attention score computed from query and key:  
\begin{align*}
T^{k}_{i,j} =
\begin{cases}
    MLP(\tau(\mathbb{SP}_{i,j}| \mathbb{A}, \mathbb{T})) & \ \textit{if} \ \ \mathbb{SP}_{i,j} \neq \emptyset \\
    -\infty & \textit{otherwise}
\end{cases}
\end{align*}
\begin{align*}
    \textit{Att}^{k} = \frac{Q^k K^k}{\sqrt{d^k}} + T^k
\end{align*}
where $\tau$ is a multi set approximator. Above equations also illustrates that our global attention mechanism can manipulate all components in the graph Fourier space, which helps to address the low-path concern (see Appendix B) in graph learning problem. After that, the PathFormer encoder layer updates the node features as the standard Transformer encoder:
\begin{align*}
    O^k &= \textit{softmax}(e^{\textit{Att}^{k}})V^k \\
    Z^{k+1} &= \textit{FFN}(O^k)
\end{align*}

\subsection{Attention interpretation machines}
In this section, we introduce our proposed interpretation machines in the PathFormer model. Specifically, the first interpretation machine is based on the proposed global attention mechanism to provide instance-level (personalized) explanation and group-level (population-based) explanation, while revealing their correlations. On the other hand, the second interpretation machine introduces trainable parameters to characterize the significance of each gene and can generate a population-based explanation. 

\textbf{Attention score based interpretation mechanism}
The first interpretation machine resorts to the framework of additive feature attribution methods, which provide explanation through a linear function of binary variables. Numerous interpretable AI models in image processing are unified in this framework and provide meaningful explanations on images. To specifically interpret graph neural networks on graph-structured data, we adapt the definition of the additive property for graph data attribution as follows: 
\begin{align*}
    \epsilon(A) = \phi_{0} + \sum \phi_{i,j} A_{i,j}
\end{align*}
where A is the adjacency matrix of the explanation, $A_{i,j}$ is a binary variable representing the existence of an edge. explanation Unlike a standard message passing GNN model, the attention matrices $\textit{Att}^{1}$...$\textit{Att}^{K}$ from our PathFormer model (where K is the number of PathFormer encoder layers) encode the pathway message information, gene profile expressions and topology information. Thus, we can interpret the K-layer PathFomer of each sample/patient as following: 
\begin{align*}
    \epsilon_{i,j} = \sum^{K}_{k=1} \textit{Att}^{k}_{i,j}
\end{align*}
Here we define the biomarkers as the genes most relevant to the prediction of the PathFormer model, which can be quantitatively measured as $e_i= \sum_{j} \epsilon_{i,j}$ . Then, to detect the core gene sub-network, we can sort $\{e_i,i \in V\}$ to detect the most relevant genes. Furthermore, as each attention matrix $\textit{Att}^{k}$ is adjusted by the pathway correlation matrix, the core gene sub-network also contains shortest pathways between selected genes to allow the pathway information aggregation. 



==> 7_future.tex <==
\zh{Currently, there could be multiple ways to implement the encoding-based downstream NAS search (i.e. sample random architecture, perturb architecture, and train predictor model, and each of them includes multiple baselines.), and there are lot's of DAG encoding frameworks (path-based, structure-based, computation-based) can serve as baselines, thus there is no enough time to have sound experimental results to include this discussion in this paper. I plan to discuss it in the future work section, and focus more on the attention-based DAG-VAE in this paper. Would it be a good choice? }

==> checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{see appendix \ref{sec:theo 3.3}}
  \item Did you discuss any potential negative societal impacts of your work?
     \answerNo{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendices \ref{sec:theo 3.2}, \ref{sec:theo 3.3}, and \ref{sec:dif}. We might include \ref{sec:theo 3.2} and \ref{sec:theo 3.3} in the Camera-ready final submission if this paper is accepted.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{see section \ref{exper}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
   \answerYes{see section \ref{exper} }
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{see Table \ref{tab: recon} and Table \ref{tab:pred} }
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
   \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{Currently the code is private.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

